Dynamic Net Metering for Energy Communities

We propose a social welfare maximizing market mechanism for an energy community that aggregates individual and community-shared energy resources under a general net energy metering (NEM) policy. Referred to as Dynamic NEM (D-NEM), the proposed mechanism dynamically sets the community NEM prices based on aggregated community resources, including flexible consumption, storage, and renewable generation. D-NEM guarantees a higher benefit to each community member than possible outside the community, and no sub-communities would be better off departing from its parent community. D-NEM aligns each member's incentive with that of the community such that each member maximizing individual surplus under D-NEM results in maximum community social welfare. Empirical studies compare the proposed mechanism with existing benchmarks, demonstrating its welfare benefits, operational characteristics, and responsiveness to NEM rates.

==> AppProofs/EffeciencyCorol_proof.tex <==
This is a straightforward result from Theorem \ref{thm:Equilibrium} and Lemma \ref{lem:CentralizedSoln}. Because the aggregate surplus of community members is equivalent to the maximum community welfare, \ie welfare under centralized operation, it holds that the maximum welfare is fully allocated (re-distributed) via D-NEM pricing mechanism to the community members. Indeed the aggregate surplus is
\begin{align*}
    \sum_{i\in \Nc} S^{\chi^\ast}_i(\psi^\ast(g_i)&,g_i) =\hspace{-0.2cm} \sum_{i\in \Nc} \Big(U_i(\bm{d}_{i}^{\psi^\ast}(\pi^\ast)) - P^{\chi^\ast}(z_{i}^{\psi^\ast}(\pi^\ast))\big)\\&\stackrel{\text{(Lem.\ref{lem:CostCausation})}}{=} \sum_{i\in \Nc} U_i(\bm{d}_{i}^{\psi^\ast}(\pi^\ast)) - P^{\mbox{\tiny NEM}}(z_{\Nc}^{\psi^\ast})\\&~~\stackrel{\text{(A)}}{=} W^\sharp,
\end{align*}
where (A) is because $\bm{d}^{\psi^\ast}_i = \bm{d}^{\sharp}_i, z^{\psi^\ast}_i = z^{\sharp}_i$, for all $i \in \Nc$.

==> AppProofs/IndRationality_Proof.tex <==
 \begin{lemma}[Individual rationality under Stackelberg equilibrium]\label{lem:IndRationality}
The surplus of every $i\in \Nc$ member under the equilibrium ($\chi^\ast,\psi^\ast$) is no less than the maximum benchmark surplus, \ie $S^\chi_i(\psi^\ast(g_i),g_i) \geq S^{\ast,\mbox{\tiny NEM}}_i(g_i)$.
 \end{lemma}

\subsubsection*{Proof of Lemma \ref{lem:IndRationality}}
We recall the active customer's surplus under the DSO's NEM X, derived in \cite{Alahmed&Tong:22IEEETSG}
\begin{align}
    S^{\ast,\mbox{\tiny NEM}}_i(g_i)= \begin{cases}   U_{i}(\bm{d}^{\pi^+}_i)-\pi^+ (\bm{1}^\top \bm{d}^{\pi^+}_i-g_i),&\hspace{-.75em} g_i< \bm{1}^\top \bm{d}^{\pi^+}_i \\ U_{i}(\bm{d}^o_i(g_i)),&\hspace{-4.7em} g_i\in [\bm{1}^\top \bm{d}^{\pi^+}_i,\bm{1}^\top \bm{d}^{\pi^-}_i] \\ U_{i}(\bm{d}^{\pi^-}_i)-\pi^- (\bm{1}^\top \bm{d}^{\pi^-}_i-g_i),&\hspace{-.75em} g_i> \bm{1}^\top \bm{d}^{\pi^-}_i,  \end{cases}\nn
\end{align}
where $\bm{d}^{\pi^+}_i, \bm{d}^{\pi^-}_i$ are as in Lemma \ref{lem:CentralizedSoln}, and $\bm{d}^o_i(g_i)$ is customer's $i$ consumption in the net-zero zone, i.e., $\bm{1}^\top \bm{d}^o_i(g_i) = g_i$ when $g_i \in [\bm{1}^\top \bm{d}^{\pi^+}_i,\bm{1}^\top \bm{d}^{\pi^-}_i]$.
Under D-NEM, the surplus of every $i \in \mathcal{N}$ community member is given by (from Lemma \ref{lem:CentralizedSoln}):
\begin{align}
    &S^{\chi^\ast}_i(\psi^\ast(g_i),g_i))=\nn\\& \begin{cases} U_i(\bm{d}_{i}^{\psi^\ast}(\pi^+)) -  \pi^+ z_{i}^{\psi^\ast}(\pi^+)&, g_\Nc<f_\Nc(\pi^+) \\ U_i(\bm{d}_{i}^{\psi^\ast}(\pi^z)) -  \pi^z z_{i}^{\psi^\ast}(\pi^z) &\hspace{-0.45cm}, g_\Nc\in[f_\Nc(\pi^+),f_\Nc(\pi^-)] \\ U_i(\bm{d}_{i}^{\psi^\ast}(\pi^-)) -  \pi^- z_{i}^{\psi^\ast}(\pi^-)&,
 g_\Nc>f_\Nc(\pi^-)\end{cases}\nn
\end{align}
which can be written as 
\begin{align}
    &S^{\chi^\ast}_i(\psi^\ast(g_i),g_i))=\nn\\& \begin{cases} U_i(\bm{d}^{\pi^+}_i) -  \pi^+ (\bm{1}^\top \bm{d}^{\pi^+}_i -g_i)&, g_\Nc<f_\Nc(\pi^+) \\ U_i(\bm{d}_{i}^{\psi^\ast}\hspace{-0.1cm}(\pi^z))\hspace{-0.1cm} -\hspace{-0.1cm}  \pi^z (\bm{1}^\top \bm{d}_{i}^{\psi^\ast}\hspace{-0.15cm}(\pi^z)\hspace{-0.05cm} -g_i) &\hspace{-0.39cm}, g_\Nc\hspace{-0.05cm}\in[f_\Nc(\pi^+),f_\Nc(\pi^-)] \\ U_i(\bm{d}^{\pi^-}_i) -  \pi^- (\bm{1}^\top \bm{d}^{\pi^-}_i -g_i)&,
 g_\Nc>f_\Nc(\pi^-)\end{cases},\nn
\end{align}
because $\bm{d}_{i}^{\psi^\ast}(\pi^+) = \bm{d}^{\pi^+}_i$ and $\bm{d}_{i}^{\psi^\ast}(\pi^-) = \bm{d}^{\pi^-}_i$ for all $i\in \Nc$. For brevity, we assume a single device case $K=1$. The proof initially assumes non-binding consumption upper and lower limits $\underline{\bm{d}}_i, \overline{\bm{d}}_i, \forall i \in \mathcal{N}$, but at the end we show how it generalizes to consumption limits inclusion. 

For every member $i \in \mathcal{N}$, the surplus difference $\Delta S_i^{\mbox{\tiny NEM},\chi^\ast}:=S^{\chi^\ast}_i(\psi^\ast(g_i),g_i))- S^{\ast,\mbox{\tiny NEM}}_i(g_i)$ expands to the following 9 pieces (\ref{subeq:case1})--(\ref{subeq:case9}).

\begin{subequations}\label{eq:DeltaSproof}
\begin{equation}\label{subeq:case1}
  0, g_\mathcal{N}<f_\Nc(\pi^+), g_i< d^{\sharp +}_i
\end{equation}    
\begin{equation}\label{subeq:case2}
  U_i(d^{\sharp +}_i)-U_i(g_i)-\pi^+\tilde{d}^{\sharp \pi^+}_i, g_\mathcal{N}<f_\Nc(\pi^+), g_i \in [d^{\sharp +}_i,d^{\sharp -}_i]
\end{equation}    
\begin{equation}\label{subeq:case3}
  U_i(d^{\sharp +}_i)-U_i(d_i^-)-\pi^+\tilde{d}^{\sharp \pi^+}_i+\pi^-\tilde{d}^{\sharp \pi^-}_i, g_\mathcal{N}<f_\Nc(\pi^+), g_i > d^{\sharp -}_i
\end{equation}    
\begin{equation}\label{subeq:case4}
  U_i(d_i^z)-U_i(d^{\sharp +}_i)-\pi^z\tilde{d}^z_i+\pi^+\tilde{d}^{\sharp \pi^+}_i, g_\mathcal{N}\in [f_\Nc(\pi^+),f_\Nc(\pi^-)], g_i< d^{\sharp +}_i
\end{equation}    
\begin{equation}\label{subeq:case5}
  U_i(d_i^z)-U_i(g_i)-\pi^z\tilde{d}^z_i, g_\mathcal{N}\in [f_\Nc(\pi^+),f_\Nc(\pi^-)], g_i\in [d^{\sharp +}_i,d^{\sharp -}_i]
\end{equation}    
\begin{equation}\label{subeq:case6}
  U_i(d_i^z)-U_i(d^{\sharp -}_i)-\pi^z\tilde{d}^z_i+\pi^-\tilde{d}^{\sharp \pi^-}_i, g_\mathcal{N}\in [f_\Nc(\pi^+),f_\Nc(\pi^-)], g_i> d^{\sharp -}_i
\end{equation}    
\begin{equation}\label{subeq:case7}
  U_i(d^{\sharp -}_i)-U_i(d_i^+)-\pi^-\tilde{d}^{\sharp \pi^-}_i+\pi^+\tilde{d}^{\sharp \pi^+}_i, g_\mathcal{N}>f_\Nc(\pi^-), g_i < d^{\sharp +}_i
\end{equation}    
\begin{equation}\label{subeq:case8}
  U_i(d^{\sharp -}_i)-U_i(g_i)-\pi^-\tilde{d}^{\sharp \pi^-}_i, g_\mathcal{N}>f_\Nc(\pi^-), g_i\in [d^{\sharp +}_i,d^{\sharp -}_i]
\end{equation}    
\begin{equation}\label{subeq:case9}
  0, g_\mathcal{N}>f_\Nc(\pi^-), g_i> d^{\sharp -}_i
\end{equation}    
\end{subequations}

where $d_i^z:= d_{i}^{\psi^\ast}(\pi^z)$ and  $\tilde{d}^{\sharp \pi^+}_i:=d^{\sharp +}_i-g_i, \tilde{d}^z_i:=d^z_i-g_i$ and $\tilde{d}^{\sharp \pi^-}_i:=d^{\sharp -}_i-g_i$ are the renewable-adjusted optimal consumptions.

We use the following property for concavity of $U(\cdot)$ 
\beq \label{eq:ConcavityPropoerty}
L(x)\geq \frac{U(y)-U(x)}{y-x}\geq L(y).
\eeq
to show that $\Delta S_i\geq 0$, by proving the non-negativity of every piece in (\ref{eq:DeltaSproof}).

--  \underline{Pieces (\ref{subeq:case1}) and (\ref{subeq:case9})}: In pieces 1 and 9, the consumption of both the community member and its benchmark are $d^{\sharp +}_i$ and $d^{\sharp -}_i$, respectively. Given that they also face the same price, their surplus difference is zero.

--  \underline{Piece (\ref{subeq:case2})}: Given that $g_i>d_i^+$, we have:
\begin{align*}
\begin{gathered}
L_i\left(d_i^{+}\right) \geq \frac{U_i\left(g_i\right)-U_i\left(d_i^{+}\right)}{g_i-d_i^{+}} \geq L_i\left(g_i\right) \\
\pi^{+}\left(d_i^{+}-g_i\right) \leq U_i\left(d_i^{+}\right)-U_i\left(g_i\right) \leq L_i\left(g_i\right) \left(d_i^{+}-g_i\right) \\
0 \leq U_i\left(d_i^{+}\right)-U_i\left(g_i\right)-\pi^{+}\tilde{d}^{\sharp \pi^+}_i \leq\left(L_i\left(g_i\right)-\pi^{+}\right)\tilde{d}^{\sharp \pi^+}_i
\end{gathered}
\end{align*}
where we used $L_i(d^{\sharp +}_i)=\pi^+$. Therefore, the surplus difference in piece (\ref{subeq:case2}) is non-negative.

\par --  \underline{Piece (\ref{subeq:case3})}: Given that $d_i^- > d_i^+$, we have:
\begin{equation*}
\pi^+(d^{\sharp +}_i-d^{\sharp -}_i)\leq U_i(d^{\sharp +}_i)-U_i(d^{\sharp -}_i)\leq \pi^- (d^{\sharp +}_i-d^{\sharp -}_i).
\end{equation*}

Using the lower bound $\pi^+(d^{\sharp +}_i-d^{\sharp -}_i)$, piece (\ref{subeq:case3}) becomes $(\pi^+-\pi^-)(g_i-d^{\sharp -}_i)\geq 0$, because $g_i> d^{\sharp -}_i$ and $\pi^+ \geq \pi^-$.

--  \underline{Piece (\ref{subeq:case4})}: Given that $d_i^+<d_i^z(g_\mathcal{N})$ (see Lemma \ref{lem:CentralizedSoln}), we have:
\begin{equation*}
\pi^+ (d_i^z(g_\mathcal{N})-d^{\sharp +}_i)\geq U_i(d_i^z(g_\mathcal{N}))-U_i(d^{\sharp +}_i)\geq \pi^z (d_i^z(g_\mathcal{N})-d^{\sharp +}_i).
\end{equation*}

Using the lower bound $\pi^z (d_i^z(g_\mathcal{N})-d^{\sharp +}_i)$, we get $(\pi^+-\pi^z)(d^{\sharp +}_i-g_i)\geq0$, because $\pi^+\leq \pi^z$ (from corollary \ref{corol:NZprice}) and $g_i<d^{\sharp +}_i$.

-- \underline{Piece(\ref{subeq:case5})}: Here, we have two cases.
\par Case 1: If $d_i^z(g_\mathcal{N})> g_i$, we have:
\begin{equation*}
L_i(g_i) (d_i^z(g_\mathcal{N})-g_i)\geq U_i(d_i^z(g_\mathcal{N}))-U_i(g_i)\geq \pi^z (d_i^z(g_\mathcal{N})-g_i),
\end{equation*}
which shows the non-negativity of piece (\ref{subeq:case5}).
\par Case 2: If $d_i^z(g_\mathcal{N})< g_i$, then
\begin{equation*}
\pi^z (g_i-d_i^z(g_\mathcal{N}))\geq U_i(g_i)-U_i(d_i^z(g_\mathcal{N}))\geq L_i(g_i) (g_i-d_i^z(g_\mathcal{N})).
\end{equation*}
By multiplying by ($-1$), we can see the non-negativity of piece (\ref{subeq:case5}).

-- \underline{Piece (\ref{subeq:case6})}: Given that $d_i^z(g_\mathcal{N})<d^{\sharp -}_i$, we have:
\begin{equation*}
\pi^z (d_i^z(g_\mathcal{N})-d^{\sharp -}_i)\leq U_i(d_i^z(g_\mathcal{N}))-U_i(d^{\sharp -}_i)\leq \pi^- (d_i^z(g_\mathcal{N})-d^{\sharp -}_i).
\end{equation*}

Using the lower bound $\pi^z (d_i^z(g_\mathcal{N})-d^{\sharp -}_i)$, we get $(\pi^z-\pi^-)(g_i-d^{\sharp -}_i)\geq0$, because $\pi^z\geq\pi^-$ and $g_i>d^{\sharp -}_i$.

--  \underline{Piece (\ref{subeq:case7})}: Given $d^{\sharp -}_i>d^{\sharp +}_i$, we have:
\begin{equation*}
\pi^+(d^{\sharp -}_i-d^{\sharp +}_i)\geq U_i(d^{\sharp -}_i)-U_i(d^{\sharp +}_i)\geq \pi^- (d^{\sharp -}_i-d^{\sharp +}_i).
\end{equation*}
Using the lower bound $\pi^- (d^{\sharp -}_i-d^{\sharp +}_i)$, we get $(\pi^+-\pi^-)(d_i^+-g_i)\geq0$, because $\pi^+\geq \pi^-$ and $d_i^+>g_i$.

--  \underline{Piece (\ref{subeq:case8})}: Given $d^{\sharp -}_i>g_i$, we have:
\begin{equation*}
    L_i(g_i)(d^{\sharp -}_i-g_i)\geq U_i(d^{\sharp -}_i)-U_i(g_i)\geq \pi^- (d^{\sharp -}_i-g_i).
\end{equation*}
The inequality $U_i(d^{\sharp -}_i)-U_i(g_i)\geq \pi^- (d^{\sharp -}_i-g_i)\geq 0$ proves that piece (\ref{subeq:case8}) is non negative, because $d_i\geq g_i$.\\
Given the non-negativity of all 9 pieces (\ref{subeq:case1})--(\ref{subeq:case9}), we have $\Delta S_i^{\pi,\chi}\geq 0$. 

Lastly, we comment on the generalization to consumption limits. Note that if $d^{\sharp +}_i = \overline{d}_i$, then we have $d^z_i= d^{\sharp -}_i = \overline{d}_i$ because of the monotonicity of the inverse marginal utility $f_i$ and $\pi^+ \leq \pi^z \leq \pi^-$. Similarly, if $d^{\sharp -}_i = \underline{d}_i$, then we have $d^z_i= d^{\sharp +}_i = \underline{d}_i$. Given that the proof of $\Delta S_i^{\pi,\chi}\geq 0$ when $d^+ = \overline{d}_i$ and $d^{\sharp -}_i = \underline{d}_i$ is trivial, it only remains to show the other cases. \hfill$\blacksquare$

==> AppProofs/NZprice_Proof.tex <==
We showed in Theorem \ref{thm:MarketEffeciency} and Lemma \ref{lem:CentralizedSoln}
that the D-NEM price $\pi^z(g_\mathcal{N}):=\mu^\ast(g_\mathcal{N})$ in the net-zero zone $g_\mathcal{N} \in [d_\mathcal{N}^+,d_\mathcal{N}^-]$ is the solution of:
 \begin{equation*}
 \sum_{i \in \mathcal{N}} \sum_{k \in \mathcal{K}} \max\{\underline{d}_{ik}, \min\{f_{ik}(\mu),\bar{d}_{ik}\}\} = g_\mathcal{N}.
\end{equation*}
By letting
\begin{equation*}
 F(x):= \sum_{i \in \mathcal{N}} \sum_{k \in \mathcal{K}} \max\{\underline{d}_{ik}, \min\{f_{ik}(\mu),\bar{d}_{ik}\}\} - g_\mathcal{N},
\end{equation*}
we note that $F(\cdot)$ is a continuous and monotonically decreasing function of $g_\mathcal{N}$. When $g_\mathcal{N} \in [d_\mathcal{N}^+,d_\mathcal{N}^-]$, we have
\[ F(\pi^+)\leq 0,\quad \quad F(\pi^-)\geq 0.\]
Therefore, there must exists $\mu \in [\pi^-,\pi^+], \text{s.t. }F(\mu)=0$. Furthermore, the continuity and monotonicity of $F(\cdot)$ in $g_\mathcal{N}$ implies that $\mu$ is a continuous and monotonically decreasing function of $g_\mathcal{N}$. \hfill$\blacksquare$

==> AppProofs/ProofsMain.tex <==
\subsection{Proof of Theorem \ref{thm:MarketEffeciency}}
\input{AppProofs/MktEff_Proof}


%%%%%%%%%%%%%% Bounded NZ zone price %%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Corollary \ref{corol:NZprice}}
\input{AppProofs/NZprice_Proof}

%%%%%%%%%%%%% Individual Rationality Thm %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem \ref{thm:MemberSurplus_Model2}}
\input{AppProofs/IndRationality_Proof}

%%%%%%%%%%%%%%%%%%%%%% Cost-Causation Principle Theorem %%%%%%%%%%%%%%%%
\subsection{Proof of Theorem \ref{thm:CausationPrinciple_Model2}}
\input{AppProofs/CostCausation_Proof}

%%%%%%%%%%%%%%%%%%%%%%%%% Group rationality %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem \ref{thm:GroupRationality}}
\input{AppProofs/GrpRationality_Proof}


